Analyzing Search Techniques for Autotuning Image-based GPU Kernels: The Impact of Sample Sizes

Modern computing systems are increasingly more complex, with their multicore CPUs and GPUs accelerators changing yearly, if not more often. It thus has become very challenging to write programs that efficiently use the associated complex memory systems and take advantage of the available parallelism. Autotuning addresses this by optimizing parameterized code to the targeted hardware by searching for the optimal set of parameters. Empirical autotuning has therefore gained interest during the past decades. While new autotuning algorithms are regularly presented and published, we will show why comparing these autotuning algorithms is a deceptively difficult task. In this paper, we describe our empirical study of state-of-the-art search techniques for autotuning by comparing them on a range of sample sizes, benchmarks and architectures. We optimize 6 tunable parameters with a search-space size of over 2 million. The algorithms studied include Random Search (RS), Random Forest Regression (RF), Genetic Algorithms (GA), Bayesian Optimization with Gaussian Processes (BO GP) and Bayesian Optimization with Tree-Parzen Estimators (BO TPE). Our results on the ImageCL benchmark suite suggest that the ideal autotuning algorithm heavily depends on the sample size. In our study, BO GP and BO TPE outperform the other algorithms in most scenarios with sample sizes from 25 to 100. However, GA usually outperforms the others for sample sizes 200 and beyond. We generally see the most speedup to be gained over RS in the lower range of sample sizes (25-100). However, the algorithms more consistently outperform RS for higher sample sizes (200-400). Hence, no single state-of-the-art algorithm outperforms the rest for all sample sizes. Some suggestions for future work are also included.

==> content/background/data-visualization.tex <==
\section{Data visualization}
When presenting a large collection of results a significant challenge is how to present the results in an intuitive and representative way, without misleading the reader. In this section we will present various data visualization types and highlight some common pitfalls in their usage.

\subsection{Heatmaps}
\iffalse
\begin{figure}\label{fig:heatmap-example}
    \centering
        \begin{subfigure}[t]{0.5\textwidth}
            \centering
            \includegraphics[width=6cm]{images/results/cles/heatmap/cles_heatmap_harris_gtx980_1.png}
            \caption{CL example with scale from 0 to 1}
        \end{subfigure}%
        ~ 
        \begin{subfigure}[t]{0.5\textwidth}
            \includegraphics[width=6cm]{images/results/rbc/rbc_heatmap_harris_gtx980_1_extra.png}
            \caption{RBC example with scale from -1 to 1}
        \end{subfigure}
        \caption{Examples of heatmaps}
    \label{fig:my_label}
\end{figure}
\fi
To more clearly visualize the magnitude of values in a two-dimensional array we can use a two-dimensional heatmap~\cite{wilkinson_history_2009}. Each value in the array is assigned a cell and the magnitude of the value will be represented as a hue on a color palette. In Fig.~\label{fig:heatmap-example} we have the pairwise CL effect size and RBC effect size of 6 algorithms. The cells colored in shades of red represent the lower end of the range and cells colored in shades of blue represent higher end of the applicable range. Since the range of CL and RBC are difference the color palette's range has been changed accordingly. This coloring makes it easier and more intuitive to find patterns in the data set.  

\subsection{KDE plots}
\iffalse
\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=4.3cm]{images/results/distributions/runtime_distribution.png}
        \caption{KDE with 800 samples}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=4.3cm]{images/results/distributions/runtime_distribution_30.png}
        \caption{KDE with 30 samples}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=4.3cm]{images/results/distributions/rf_25_100_775.png}
        \caption{KDE with 25, 100, 775 samples}
        \label{fig:KDE-example-25-100-775}
    \end{subfigure}
    \caption{Comparison of KDEs at varying sample sizes}
    \label{fig:KDE-example}
\end{figure}
\fi
When we have a large collection of samples and we want to visualize the density of samples dependent on some variable $X$ a natural tool is the \emph{histogram}. However, as the sample size grows and the width of the histograms shrink we approximate a continuous density curve. One way to calculate and visualize such a density curve is Kernel Density Estimation(KDE). In Fig.~\ref{fig:KDE-example} we can see two examples of histograms and their respective KDE for various sample sizes. 

We can also see in Fig.~\ref{fig:KDE-example-25-100-775} that the form of the KDE can change significantly as we change the sample sizes. A KDE with a low number of samples can therefore be deceiving, since the KDE does not give any indication to how the representativeness the KDE is of the true distribution. A KDE should therefore ideally include a confidence interval in the visualization, however to the author's knowledge data visualization libraries for python do not support this yet. A countermeasure is therefore to ensure that the KDE is given sufficient examples to as not to be misleading, and clearly warn the reader when it is not feasible to produce more samples.


\subsection{Violin plots}
\iffalse
\begin{figure}
    \centering
    \includegraphics[width=7cm]{images/results/distributions/violin_example.png}
    \caption{Example of violin plot}
    \label{fig:violin-example}
\end{figure}
\fi
By combining a KDE plot with a box plot, we get the very information dense \emph{violin} plot. This allows us to compactly compare the distribution of samples, together with their minimum, first quartile, median, third quartile and maximum values. In Fig.~\ref{fig:violin-example} we compare three different algorithms that have similar median values, but significantly different density distributions, interquartile range and maximum values.
    
\subsection{Libraries}
While the most common library for data visualization in Python is \emph{matplotlib} there are many supporting libraries that improve upon the library. One of these libraries is \emph{Seaborn} which provides a wide range of standardized color palettes and formating schemes to create consistency and improve interpretability of the plots.

==> content/background/docker-and-reproducibility.tex <==
\section{Docker and Reproducibility}
To ensure a good empirical study we need to ensure that our results are \emph{falsifiable}. To enable this, we need to ensure that all of our source code, data, hardware, runtime environment, and any other significant factors are described in detail. The study then needs to be \emph{reproducible}, where most studies do not publish any code, nor the necessary configuration to get the program running, \emph{Docker} allows us to easily ensure a reproducible test environment.

Docker is a virtualization technology for Linux that encapsulates runtime dependencies and libraries on an OS-level as \emph{containers}. Given a Docker \emph{image} and similar hardware a researcher can use a provided image to create a container with an identical runtime environment as the original study. This image can then be used on many different architectures and operating systems without changing the runtime environment of the container.   

\subsection{Nvidia-docker}
While Docker supports running on many CPU architectures like x86 and POWER9 processors, docker initially had no direct support for running applications on GPUs. Nvidia thus developed \emph{nvidia-docker} as a solution to run CUDA programs from within a Docker container. To enable this developers need to use the nvidia's own development of docker and the Docker images need to be based on nvidia's compatible images, like their CUDA image~\footnote{nvcr.io/nvidia/cuda}. Nvidia also supports running OpenCL programs using their OpenCL image~\footnote{nvcr.io/nvidia/opencl}.

==> content/background/gpu-introduction.tex <==
\subsection{GPU Architecture}
\iffalse
\begin{figure}
    \centering
    \includegraphics[width=10cm]{content/background/gpu-vs-cpu.png}
    \caption{Illustration for the relative sizes of various logic circuits on CPUs vs GPUs, with permission from NVIDIA.}
    \label{fig:cpu-vs-gpu}
\end{figure}
\fi

GPUs are based on a Single Instruction Multiple Data(SIMD) model, where many processing elements perform the same instruction on a large collection of different data. This model enables the hardware to greatly reduce the size of control logic and caching for the processing elements. Designers can reduce the complexity of branch predictors and share a front-end across many cores, so as to optimize die area for purely computational resources (See Fig.~\ref{fig:cpu-vs-gpu}). This comes at a reduced single-core performance and increased latency; however it greatly increases the throughput for workloads that are sufficiently parallelized. 

\iffalse
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=5cm]{content/background/grid-of-thread-blocks.png}
        \subcaption{Illustration for organization of threads, with permission from NVIDIA.}
        \label{fig:grid-of-thread-blocks}
    \end{subfigure}%
    ~
    \begin{subfigure}[b]{0.6\textwidth}
        \centering
        \includegraphics[width=7cm]{content/background/memory-hierarchy.png}
        \subcaption{Illustration of the memory hierarchy, with permission from NVIDIA.}
        \label{fig:memory-hierarchy}
    \end{subfigure}
    \caption{Illustration of execution and memory hierarchy in the CUDA programming model, with permission from NVIDIA.}
    
\end{figure}
\fi

This produces a hardware design with hundreds or thousands of cores that execute in lockstep. Using Nvidia's terminology~\cite{nvidia_nvidia_nodate} these cores are programmed using a \emph{grid} that subdivides thousands of \emph{threads} into \emph{blocks}, see Fig.~\ref{fig:grid-of-thread-blocks}. Each block executes its threads as \emph{warps} of 32 threads that execute in lock-step on a \emph{streaming processor}(SP). Each block is assigned a \emph{streaming multiprocessor}(SM) that can include several SPs. The memory hierarchy of this architecture is described in Fig.~\ref{fig:memory-hierarchy}, where all of these SPs have access to a fast shared \emph{global memory}. Additionally the cores in the same SM have access to a \emph{scratchpad memory} that can be programmatically assigned to or dynamically used as cache. Lastly each thread can individually read and write from the register file. 

\subsection{OpenCL}
With a wide range of architectures and different computing models it gets increasingly difficult for developers to produce programs that run well on any architecture. OpenCL~\cite{stone_opencl_2010} was therefore created as an Open standard for computation on any architecture. The goal is thus to create a programming model where the code can be written once and executed anywhere, from CPUs to GPUs and FPGAs. The programming model is quite similar to CUDA and has therefore gotten significant support from both AMD and Nvidia as an open alternative to CUDA. OpenCL is still under development and currently contains many parameters such as \emph{work group size}(similar to the size of the threadblock in CUDA), that needs to be tuned for each architecture to provide optimal performance. So OpenCL promises \emph{functional portability}, but gives no guarantees of \emph{performance portability}. 

\subsection{Performance Portability}
Due to the wide range of hardware available for computers, a program will often \emph{functionally} behave the same for all compatible platforms, however the \emph{performance} can vary greatly. A configuration of a problem that runs well on a CPU might perform terribly for a GPU. When writing high-performance software, it is important that we utilize the hardware as efficiently as possible, which is why ATLAS~\cite{clint_whaley_automated_2001} was created. ATLAS is an Automatically Tuned Linear Algebra library, where the executing hardware determines the libraries' configuration. It does this by testing out various configurations to determine what configuration is optimal for this specific hardware. One way to do this is by analysing the size of the cache levels and using this data to determine optimal compute sizes. Using these automatic techniques, we can avoid the manual labor of finding the optimal configuration for every single hardware platform. FFTW~\cite{frigo_fftw_1998} used a similar concept of self-tuning to optimize its fast fourier transforms.


==> content/results/medians-charts.tex <==

%For many of our results the margins are quire narrow, which necessitate more careful study in Section~\ref{sec:stats-p-value} to measure if these results are statistically significant. 
%The Non-SMBO method RF underperform compared with the SMBO-methods and RS for most of the benchmarks and architectures. 
%The exception is AUMAs strong performance for low sample sizes on a selection of benchmarks and architectures. We suspect that AUMAs performance is due to strong overfitting or underfitting. 

%\subsection{Statistical significance}\label{sec:stats-p-value}
%When we present these results we need to ensure that they are \emph{statistically significant}, i.e. when we present that one algorithm outperforms another, do have sufficient evidence for this conclusion? 
%Using the experimental design specified in Chapter~\ref{chap:method}, we will now present our analysis of these significance results. 
%The full significance tests are available in Appendix~\ref{apx:p-value-heatmaps} as heatmaps. 
%We also discuss the necessity of a high number of experiments due to fluctuations in p-value as a function of experiment size in Appendix~\ref{apx:p-value-evolution}.

%For sample size 25 BO GP, BO TPE or AUMA are the optimal solution, depending on the benchmark and architecture. We don't provide p-values for Titan V results, since these are only preliminary results without AUMA. 
%BO GP is better than all others for this sample size for all GTX 980 and RTX Titan benchmarks and architecture combinations except for Harris on RTX Titan and Add on GTX 980 where AUMA outperforms and Mandelbrot on the GTX 980 where BO TPE outperforms. 
%Our preliminary results also indicate that BO TPE outperforms all others for the Harris benchmark on the Titan V.

%For sample size 50, BO GP is the optimal solution for all cases, with very strong p-values, with the closest exception being the Mandelbrot benchmark on the GTX 980 ($p=0.0031$).

%For sample size 100, BO GP is the optimal solution for all cases except for Harris benchmark on the RTX Titan(Fig.~\ref{fig:normalized-median-harris-rtx-titan}) and the Mandelbrot benchmark on the GTX 980(where BO TPE outperforms). 
%In the case of Harris on RTX Titan we \emph{do not} have conclusive evidence for GA or BO GP being the optimal solution (p-values of $0.55$ and $0.45$ respectively).

%For sample size 200, GA performs the best for the Add benchmark and Harris benchmark, however the results are not conclusive for Harris with GTX 980(Fig.~\ref{fig:normalized-median-harris-gtx-980}) with respect to BO TPE, with a $p-value = 0.019 > \alpha$. For the Mandelbrot benchmark, BO GP performs best, however here as well the p-values are insufficient with respect to BO TPE and GA for the RTX Titan and the GTX 980.

%For sample size 400, GA appears to outperform all other algorithms for all benchmarks and architectures, except for Mandelbrot on the GTX 980 where BO GP outperforms(Fig.~\ref{fig:normalized-median-mandelbrot-gtx-980}).

%When presenting and analysing these p-values, it is important to note that high p-values in our case relate to small differences in performance. We will therefore now look at the \emph{effect size} of these differences using the Common Language effect size.

%\subsection{Optimal improvement over RS}
%In this section we plot the \emph{optimal} improvement over RS for each benchmark and architecture. These results can be seen in Fig.~\ref{fig:optimal-improvement-add}-\ref{fig:optimal-improvement-all}. Here we have taken the best performing algorithm for a specific sample size and compared it to RS. This then creates a plot for the percentage improvement over RS for each sample size for all benchmark and architecture combinations. This plot provides novel insight into how model-based approaches scale with sample sizes relative to RS. We notice that the percentage improvements over RS are largest for small sample sizes and steadily decrease as the sample sizes increases. We therefore have strong motivations to focus future research on small samples sizes, where there is most percentage improvement to be gained over RS. There is also a clear trend that simple benchmarks like Add(Fig~\ref{fig:optimal-improvement-add}) can give higher relative performance increases over RS for low sample sizes, then more complex benchmarks like Mandelbrot (Fig~\ref{fig:optimal-improvement-mandelbrot}).



%In these plots, we can also see that BO TPE performs well for sample size 25.
%, and outliers like constraint-less AUMA that perform well for very low sample sizes for a selection of algorithms and benchmarks degrade as the sample size increases. 
%Similarly, RF performs worse than RS for some benchmarks and better for others.


==> content/results/medians-effect-size.tex <==



==> content/results/medians-p-values.tex <==



==> docsetup.tex <==
%\usepackage{setspace}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{color}
\usepackage{listings}
\usepackage{subcaption}
\usepackage{authblk}
\usepackage{xcolor}
\usepackage{mathtools}
\usepackage{mathptm}
\usepackage[T1]{fontenc}
\usepackage[pdftex,bookmarks=true]{hyperref}
\usepackage[pdftex]{hyperref}
\usepackage{float}

\usepackage{setspace}
\usepackage{enumitem}
\usepackage{booktabs}
%\usepackage[Lenny]{fncychap}
\usepackage{natbib}
\usepackage[font=small,labelfont=bf]{caption}
%\usepackage{fancyhdr}
\usepackage{times}

\usepackage[utf8]{inputenc}
\usepackage{babel}
\usepackage{textcomp}
\usepackage{type1cm}
\usepackage{amsfonts}
\let\labelindent\relax

\hypersetup{
    colorlinks,%
    citecolor=black,%
    filecolor=black,%
    linkcolor=black,%
    urlcolor=black
}
%\usepackage[font=small,labelfont=bf]{caption}
%\usepackage{fancyhdr}
%\usepackage{times}
%\usepackage[intoc]{nomencl}
%\renewcommand{\nomname}{List of Abbreviations}
%\makenomenclature
%\usepackage{natbib}
%\floatstyle{boxed} 
\restylefloat{figure}
\lstset{
    language=C,                             % Code langugage
    basicstyle=\ttfamily,                   % Code font, Examples: \footnotesize, \ttfamily
    keywordstyle=\color{OliveGreen},        % Keywords font ('*' = uppercase)
    commentstyle=\color{gray},              % Comments font
    numbers=left,                           % Line nums position
    numberstyle=\tiny,                      % Line-numbers fonts
    stepnumber=1,                           % Step between two line-numbers
    numbersep=5pt,                          % How far are line-numbers from code
    frame=none,                             % A frame around the code
    tabsize=2,                              % Default tab size
    captionpos=b,                           % Caption-position = bottom
    breaklines=true,                        % Automatic line breaking?
    breakatwhitespace=false,                % Automatic breaks only at whitespace?
    showspaces=false,                       % Dont make spaces visible
    showtabs=false,                         % Dont make tabls visible
    morekeywords={__global__, __device__},  % CUDA specific keywords
}

\definecolor{darkgreen}{rgb}{0.18,0.54,0.34}
\lstset{ 
  language=C,                % the language of the code
  basicstyle= \footnotesize,           % the size of the fonts that are used for the code
  numbers=left,
  numberfirstline=true,
  numbersep=5pt,                  % how far the line-numbers are from the code
  backgroundcolor=\color{white},      % choose the background color. You must add \usepackage{color}
  showspaces=false,               % show spaces adding particular underscores
  showstringspaces=false,         % underline spaces within strings
  showtabs=false,                 % show tabs within strings adding particular underscores
  frame=lrb,                   % adds a frame around the code
  rulecolor=\color{black},        % if not set, the frame-color may be changed on line-breaks within not-black text 
  tabsize=2,                      % sets default tabsize to 2 spaces
  captionpos=t,                   % sets the caption-position 
  breaklines=true,                % sets automatic line breaking
  breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
  %title=\lstname,                   % show the filename of files included with \lstinputlisting;
  keywordstyle=\color{blue},          % keyword style
  commentstyle=\color{gray},       % comment style
  stringstyle=\color{darkgreen},         % string literal style
  escapeinside={\%*}{*)},            % if you want to add LaTeX within your code
  morekeywords={*, ..., __global__, __device__, threadIdx, method_t},               % if you want to add more keywords to the set
  xleftmargin=0.2in, % left horizontal offset of caption box
  xrightmargin=-.03in % right horizontal offset of caption box
}

% ShareLaTeX does not support glossaries now. Sorry...
%\usepackage[number=none]{glossary}
%\makeglossary
%\newglossarytype[abr]{abbr}{abt}{abl}
%\newglossarytype[alg]{acronyms}{acr}{acn}
%\newcommand{\abbrname}{Abbreviations} 
%\newcommand{\shortabbrname}{Abbreviations}
%%\makeabbr

